MedAutoCorrect: Image-Conditioned Autocorrection in Medical Reporting

In medical reporting, the accuracy of radiological reports, whether generated by humans or machine learning algorithms, is critical. We tackle a new task in this paper: image-conditioned autocorrection of inaccuracies within these reports. Using the MIMIC-CXR dataset, we first intentionally introduce a diverse range of errors into reports. Subsequently, we propose a two-stage framework capable of pinpointing these errors and then making corrections, simulating an \textit{autocorrection} process. This method aims to address the shortcomings of existing automated medical reporting systems, like factual errors and incorrect conclusions, enhancing report reliability in vital healthcare applications. Importantly, our approach could serve as a guardrail, ensuring the accuracy and trustworthiness of automated report generation. Experiments on established datasets and state of the art report generation models validate this method's potential in correcting medical reporting errors.

==> preamble.tex <==
%
% --- inline annotations
%
% \usepackage[dvipsnames]{xcolor}
% \newcommand{\red}[1]{{\color{red}#1}}
% \newcommand{\todo}[1]{{\color{red}#1}}
% \newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sup_files/analysis.tex <==
\section{Detailed Analysis}
\label{sec:dis_analysis}

\textbf{Error Detection Module: }
In our paper, we detailed the precision, recall, and F1 score for the error detection module, utilizing various error identification approaches. We extend the analysis in table~\ref{tab:model_eval_full}. Additionally, we present quantitative results that examine the impact of varying error thresholds on the Natural Language Generation (NLG) metrics of reports that have undergone autocorrection in table~\ref{tab:error_thresholds}.


\textbf{Impact of Variable Threshold Settings:} Table~\ref{tab:error_thresholds} highlights how the choice of an error threshold critically affects our model's performance. This threshold determines the confidence level required for the error detection module to classify a token as erroneous. Unlike standard binary classification where a 0.5 threshold is common, we experimented with various thresholds. A lower threshold, such as 0.6, results in under-detection of errors, thereby constraining the error correction module's scope. On the other hand, higher thresholds (0.9 or 1.0) tend to over-flag tokens, which could inadvertently lead to the introduction of new errors during `correction' of incorrectly flagged tokens and impact the overall natural language generation metrics negatively. We found a 0.7 threshold to be optimal, effectively balancing error detection accuracy and correction capabilities while preserving the linguistic coherence of the generated text.


\begin{table*}
    \centering
    \resizebox{\textwidth}{!}{\begin{tabular}{lcccccccccccc}
    
        \toprule
        & \multicolumn{3}{c}{\textbf{Patch Approach}} & \multicolumn{3}{c}{\textbf{Pool Approach}} & \multicolumn{3}{c}{\textbf{Concatenate Approach}} \\
        \cmidrule{2-10}
        & \textbf{Precision} & \textbf{Recall} & \textbf{F1-score} & \textbf{Precision} & \textbf{Recall} & \textbf{F1-score} & \textbf{Precision} & \textbf{Recall} & \textbf{F1-score} \\

        \midrule
        Error & \cellcolor{gray!25}\textbf{0.4931} & \cellcolor{gray!25}0.8763 & \cellcolor{gray!25}\textbf{0.6311} & 0.4862 & 0.8569 & 0.6204 & 0.4647 & \textbf{0.9020} & 0.6134 \\
         No Error & 0.9668 & \textbf{0.8000} & \textbf{0.8755} & 0.9617 & 0.7990 & 0.8728 & \textbf{0.9725} & 0.7693 & 0.8591 \\
        Macro Avg & \cellcolor{gray!25}\textbf{0.7300} & \cellcolor{gray!25}\textbf{0.8381} & \cellcolor{gray!25}\textbf{0.7533} & 0.7240 & 0.8279 & 0.7466 & 0.7186 & 0.8357 & 0.7362\\
        % Micro Avg & \cellcolor{gray!25}\textbf{0.7599} & \cellcolor{gray!25}\textbf{0.8400} & \cellcolor{gray!25}\textbf{0.7899} & 0.7501 & 0.8300 & 0.7801 & 0.7402 & 0.8500 & 0.7702\\
        Weighted Avg & \cellcolor{gray!25}\textbf{0.8807} & \cellcolor{gray!25}\textbf{0.8139} & \cellcolor{gray!25}\textbf{0.8311} & 0.8753 & 0.8095 & 0.8270 & 0.8803 & 0.7934 & 0.8144 \\
        \bottomrule
        Overall Accuracy & \multicolumn{3}{c}{\cellcolor{gray!25}\textbf{0.8139}} & \multicolumn{3}{c}{0.8095} & \multicolumn{3}{c}{0.7934} \\
        \bottomrule
    \end{tabular}}
    \caption{\textbf{Detailed Error Detection Results: } Evaluation of the error detection module here is done at an error sensitivity threshold of 0.7. }

    \label{tab:model_eval_full}
\end{table*}



\begin{table*}[ht!]
    \centering
    \begin{tabular}{lcccccc}
        \toprule
        & Thresholds & \textbf{BLEU-4} & \textbf{METEOR} & \textbf{ROUGE-L F1} \\
        \midrule
        Baseline & & 0.091 & 0.139 & 0.227 \\
        \midrule
       
       \multirow{1}{*}{Patch approach} & \multirow{3}{*}{0.6} & 0.104 & 0.176 & 0.295 \\
       
       \multirow{1}{*}{Pool approach} & &  0.094 & 0.145 & 0.273 \\
       
        \noalign{\vskip1pt}

        \multirow{1}{*}{Concatenate approach}& & 0.095 & 0.149 & 0.279 \\
        
        \bottomrule
       \multirow{1}{*}{Patch approach} & \multirow{3}{*}{0.7} & 0.169 & \textbf{0.204} & 0.354 \\
       
       \multirow{1}{*}{Pool approach} & &  0.152 & 0.179 & 0.338 \\
       
        \multirow{1}{*}{Concatenate approach}& & 0.150 & 0.178 & 0.337 \\
        
        \bottomrule

       \multirow{1}{*}{Patch approach} & \multirow{3}{*}{0.8} & \textbf{0.189} & 0.176 & 0.290 \\
       
       \multirow{1}{*}{Pool approach} & &  0.161 & 0.124 & 0.256 \\
       
        \multirow{1}{*}{Concatenate approach}& & 0.210 & 0.189 & 0.314 \\
        
        \bottomrule

       \multirow{1}{*}{Patch approach} & \multirow{3}{*}{0.9} & 0.171 & 0.139 & 0.241 \\
       
       \multirow{1}{*}{Pool approach} & &  0.157 & 0.173 & \textbf{0.365} \\
       
        \multirow{1}{*}{Concatenate approach}& & 0.135 & 0.196 & 0.333 \\
        
        \bottomrule
    \end{tabular}
\caption{\textbf{Impact of Different Error Sensitivity Thresholds on Error Correction Performance}. The primary analysis in the main paper (table~\ref{tab:first_eval}) utilizes a threshold of 0.7 for error detection. We extend that analysis by presenting the outcomes associated with various other error sensitivity thresholds.}

    \label{tab:error_thresholds}
\end{table*}

\begin{table*}[ht!]
    \centering
    \small
    \resizebox{\textwidth}{!}{\begin{tabular}{lclccccc|ccc}
        \toprule
        \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{6}{c|}{NLG Metrics} & \multicolumn{3}{c}{CE Metrics} \\
        & & \textbf{BL-1} & \textbf{BL-2} & \textbf{BL-3} & \textbf{BL-4} & \textbf{MTR} & \textbf{RG-L}  & P & R & F1 \\
        \midrule
        \multirow{3}{*}{\rotatebox[origin=c]{0}{MIMIC-CXR}} & Uncorrected retrieval (Ours) & 0.216 &0.108 & 0.056 & 0.029 & 0.051 & 0.187 & 0.192 & 0.173 & 0.183 \\
        & Autocorrection (Patch)  & \cellcolor{gray!25}0.370 & \cellcolor{gray!25}0.234 & \cellcolor{gray!25}0.175 & \cellcolor{gray!25}0.125 & \cellcolor{gray!25}0.112 & \cellcolor{gray!25}0.230 & \cellcolor{gray!25}0.263 & \cellcolor{gray!25}0.444  & \cellcolor{gray!25}0.330\\
        & Autocorrection (Pool)  & 0.299 & 0.202 & 0.139 & 0.121 & 0.109 & 0.205 & 0.219 & 0.446 & 0.294\\
        & Autocorrection (Concatenate)  & 0.314 & 0.231 & 0.154 & 0.118 & 0.113 & 0.227 & 0.249 & 0.431  & 0.316\\
        

        \bottomrule
    \end{tabular}}
    \caption{\textbf{Comparative Analysis of Autocorrection Approaches on retrieval model performance.} We provide an ablation study highlighting the impact of different autocorrection methods (Patch, Pool, and Concatenate) on Natural Language Generation (NLG) and Clinical Efficacy (CE) metrics against the uncorrected retrieval baseline to illustrate the improvement in report quality post-autocorrection. See figure~\ref{fig:retrieval_example} and ~\ref{fig:retrieval_2} for limitations.}
    \label{tab:second_eval}

\end{table*} 

\textbf{Limitations and Qualitative Analysis: } Figures \ref{fig:retrieval_2} and \ref{fig:attention_maps_all} provide a detailed analysis and highlight the limitations of our framework, especially in handling errors introduced by retrieval-based models or those in the test set. As discussed in Section~\ref{sec:retrieval} of the main paper, we introduce this approach as a means to mitigate retrieval errors. However, as demonstrated in Figures~\ref{fig:retrieval_example} and ~\ref{fig:retrieval_2}, the effectiveness of autocorrection is intrinsically linked to the accuracy of the underlying retrieval model. The framework's performance is constrained by the retrieval model's propensity to either over-retrieve or under-retrieve relevant information. Consequently, our autocorrection system, while robust in correcting the content it receives, is not designed to independently assess the relevance or necessity of the information within the broader clinical context. This insight opens avenues for future enhancements, particularly in integrating our autocorrection system with advanced radiology report generation modules. We advocate for researchers in report generation to explore the potential benefits of combining our autocorrection approach with their models for improved accuracy and context sensitivity.

For a comprehensive understanding of the autocorrection framework's performance, including its successes and limitations in detecting and correcting errors within text, we recommend referring to Figure~\ref{fig:attention_maps_all}. This figure provides illustrative examples that showcase the framework's capabilities and constraints in various error correction scenarios. For additional examples and failure cases, watch the video attached in the supplementary materials.

==> sup_files/error_injection.tex <==
\clearpage
\setcounter{page}{1}
\textbf{Supplementary Material }
        
\section{Discussion on Error Injection }
\label{sec:rationale}

In Section~\ref{sec:error_injection}, we briefly introduced a method for intentionally injecting errors into MIMIC-CXR reports to create the training dataset. This section aims to provide a more profound understanding of the error categories we chose, the rationale behind these choices, and the implications of these errors in clinical practice. 

\begin{wrapfigure}{r}{0.4\textwidth}
\centerline{\includegraphics[width=.4\textwidth]{sup_files/proportion.png}}
\caption{Distribution of Different Error Types in Reports Prior to Implementing the General Prompt Approach. See Section~\ref{sec:error_injection} for the details on each error type.}
\label{fig:graph}
\end{wrapfigure}


\textbf{Rationale for Error Types Selection: }
Error types were selected based on their potential for prevalence in clinical settings and their potential impact on patient care. Misdiagnoses, incorrect localization of conditions, and over or underestimation of medical findings are common issues in radiological reports and can lead to significant clinical consequences. We wanted to simulate these errors to study their effects and develop methods to detect and correct them. However, since manually injecting errors into the MIMIC-CXR reports would be a tedious process given how many they are, we decided to use an LLM with specific instructions regarding how to alter the reports.  Using OpenAI's GPT-4, we developed prompts that would lead the model to introduce specific types of errors in the radiological reports from the MIMIC-CXR dataset. The prompts were designed to reflect what goes on during radiological reporting, ensuring that the errors introduced were realistic and clinically relevant.


\textbf{Error Injection Using GPT-4: }
The GPT-4 model was prompted with segments of real radiological reports followed by instructions to alter them by introducing specific types of errors. This approach allowed us to generate a wide range of error examples that could be used for training and evaluation of our error detection and correction algorithms. The choice of GPT-4 as the LLM of choice and not other LLMs was motivated by the desire to have the model accurately place curly braces around the errors introduced at precisely the right locations. We also manually adjusted incorrectly placed curly braces in some reports to be specifically around the errors introduced. 

Initially, we aimed to generate specific error types in radiological reports using tailored prompts. However, due to high operational costs, our strategy shifted towards a more general prompt approach, as depicted in figure~\ref{fig:prompt}. This change inevitably led to a broader range of error types being introduced, impacting our ability to provide detailed, error-type-specific qualitative analysis. Consequently, our results, presented in table~\ref{tab:first_eval}, encompass a spectrum of error types. The figure~\ref{fig:graph} illustrates the distribution of error types generated prior to adopting the general prompt methodology. Below are the prompts we used to introduce specific error types. 

\begin{wrapfigure}{r}{0.4\textwidth}
\centerline{\includegraphics[width=.4\textwidth]{sup_files/sup1.pdf}}
\caption{General Prompt Structure for Error Injection in Radiological Reports. We add ``This is for a machine learning project focusing on the detection and correction of errors in radiological reports.'' to avoid responses from GPT-4 that directed to the safety concerns that come with altering medical reports}
\label{fig:prompt}
\end{wrapfigure}

\begin{enumerate}
    \item \textbf{False Prediction Prompt:} ``Given the report excerpt `\{...\}', modify it to include an erroneous condition that is not present in the original report.''
    \item \textbf{Mislocation Error Prompt:} ``Alter the report `\{...\}' to incorrectly specify the location of a reported finding.''
    \item \textbf{Severity Misjudgment Prompt:} ``Revise the report `\{...\}' to either exaggerate or downplay the severity of a condition.''
\end{enumerate}


To all of these prompts we appended ``Wrap each erroneous token or
phrase introduced in curly braces.'' so that we could keep track of where the errors had been introduced. The curly braces are removed during training and testing. We do manual post-processing to remove any additional information included by the LLM that is not related to the report. To ensure our injected errors mirror real-world inaccuracies, we consulted clinical guidelines and common error patterns identified in medical literature along with common errors in report generation models and finally did a
manual check on the dataset to confirm realism. See figure~\ref{fig:all} for a sample range of error types that make up the dataset.

\textbf{Dataset Expansion and Refinement: }Initially, we randomly sampled 30,000 reports from the MIMIC-CXR dataset, creating two distinct erroneous versions for each report, constrained by budget limitations. However, to encompass a broader range of scenarios, we expanded our sampling to include over 100,000 reports. Following rigorous post-processing and the elimination of reports with unrealistic errors, we refined our dataset to 120,123 high-quality erroneous reports. These reports effectively represent a diverse array of potential clinical errors. See fig~\ref{fig:all}.



\begin{figure*}
\centerline{\includegraphics[width=1.2\textwidth]{sup_files/sup2.pdf}}
\caption{Overview of varied error types in radiological reports, as altered via GPT-4 prompts. Top-left focuses on false predictions, top-right on mislocations, and the bottom on severity misjudgments, illustrating common error types in clinical radiology and their potential impacts on diagnostic accuracy. Some reports in the dataset consist of a mixture of errors.}
\label{fig:all}
\end{figure*}



==> sup_files/method.tex <==
\section{Discussion on Method and Training}
\label{sec:dis_meth}
\textbf{Dataset Overview: }Our training methodology for error detection involved the use of image/erroneous report pairs and image/ground truth report pairs from the MIMIC-CXR dataset which make up the full training dataset. The MIMIC-CXR dataset comprises 377,110 chest X-ray images and 227,835 free-text radiology reports. We utilized the MIMIC-CXR-JPG v2.0.0 dataset\footnote{Johnson, A., Lungren, M., Peng, Y., Lu, Z., Mark, R., Berkowitz, S., \& Horng, S. (2019). MIMIC-CXR-JPG - chest radiographs with structured labels (version 2.0.0). PhysioNet. https://doi.org/10.13026/8360-t248.}, a JPG-formatted subset of the original collection, to enhance image handling and processing efficiency. Emphasizing a diverse training strategy, we used both frontal and lateral X-ray views.

\textbf{Training Approach:} For the error detection module, we adopted a two-stage training process to address class imbalance caused by a surplus of non-erroneous tokens. Initially, we focused solely on image/erroneous report pairs for 20 epochs, enabling the model to learn error patterns effectively. Subsequently, we included image/ground truth report pairs in the training for an additional 5 epochs. This sequential training approach, prioritizing error pattern recognition followed by exposure to correct instances, proved more effective than other training configurations. Focal loss was utilized to further mitigate class imbalance issues (as mentioned in the main paper). The error correction module was trained for 800 epochs, on the dataset consisting of both image/erroneous report pairs and image/ground truth report pairs. We employed the AdamW optimizer for both modules setting the learning rate at \(3 \times 10^{-4}\).

\begin{figure*}
\centerline{\includegraphics[width=1.\textwidth]{sup_files/v.pdf}}
\caption{\textbf{Challenges in Autocorrection of Retrieved Reports (See figure~\ref{fig:retrieval_example}):} This figure highlights a significant challenge in autocorrecting retrieval-based radiology reports. It showcases instances where reports, while accurately retrieved, include additional details that are not pertinent to the current diagnosis (highlighted in yellow). These extraneous segments, although potentially relevant, deviate from the ground truth and are not efficiently identified or removed by the autocorrect system. This limitation underscores the need for enhanced discernment capabilities in the framework to differentiate between essential and non-essential information in the context of clinical diagnosis. Beyond that, autocorrection happens just as it would as illustrated in Figure~\ref{fig:attention_maps_all}}
\label{fig:retrieval_2}
\end{figure*}


\textbf{Model Architecture and Embedding Strategy:} For the image encoder, we selected the Vision Transformer (ViT), specifically the ViT-B/16 (\texttt{vit\_base\_patch16\_224})\footnote{https://github.com/huggingface/pytorch-image-models/blob/main/timm/models/vision\_transformer.py} configuration from the \texttt{timm}\footnote{https://github.com/huggingface/pytorch-image-models} library, fine-tuned on JPG chest X-rays from the MIMIC-CXR dataset. This configuration divides each image into patches of 16x16 for detailed analysis. In conjunction with ViT, we used GatorTron medium for text encoding, producing token embeddings with a dimension of 2560. These embeddings are then projected to a dimension of 1024 to align with the 768-dimensional image patch embeddings, which are also projected to 1024. This projection facilitates the alignment of image patch embeddings with the token embeddings, essential for the effective conditioning of our error detection module as mentioned in Section~\ref{sec:detection} Our preliminary experiments demonstrated the effectiveness of fine-tuning the GPT-2 model to incorporate both textual and visual information compared to GatorTron medium. GatorTron-medium however performed better in error detection, so we maintained it for that. Our custom split applied to the error-injected dataset was primarily for internal validation purposes which we report in tables ~\ref{tab:model_evaluation_with_support} and ~\ref{tab:first_eval}. The evaluation of our autocorrection framework when applied to retrieval models, utilized the official MIMIC-CXR testing set

\textbf{Inference: } In the inference stage of our correction model as mentioned in the paper, we utilize both beam search and nucleus sampling to handle corrections of varying lengths in the generated text. Beam search is an algorithm that efficiently navigates through potential sequences, considering multiple paths (beams) simultaneously, while nucleus sampling selects the next token from a subset of most likely options. Beam search, with a width of 5 beams, is employed for generating text, which helps in maintaining a balance between exploration of different possibilities and computational efficiency. This is complemented by nucleus sampling, where we set the top\_p parameter to 0.92, enabling the model to sample from the top 92\% of the probability distribution, thus providing a more diverse and contextually relevant set of predictions. This combination of beam search and nucleus sampling ensures that our model can effectively generate accurate and varied corrections for the identified errors.

We refer you to the code for more implementation details and choices.

\textbf{Training Retrieval Model:} The retrieval model, integral for evaluating the medical autocorrection framework, was developed with a specific focus on showcasing the autocorrection mechanism's effectiveness. We use the same image and text encoders we use for encoding the images and reports in the error detection and erorr correction module. It's important to note that this model was not designed for state-of-the-art (SOTA) performance in radiological report generation. The model is trained on the MIMIC-CXR dataset using a contrastive loss function, specifically tailored for image and the full ground truth report pairs. For further insights into retrieval models in radiology report generation, we recommend reviewing related literature in this field. The training was conducted for 10 epochs using a batch size of 64. This relatively short training duration is chosen to reflect the model's purpose as a tool for demonstrating autocorrection capabilities, rather than achieving peak performance metrics. The retrieval model produced errors similar to those in our dataset.

\textbf{Utilizing FAISS\footnote{https://github.com/facebookresearch/faiss} for Efficient Report Retrieval:} For the retrieval of the most relevant medical report corresponding to each image, we employ the FAISS (Facebook AI Similarity Search) library, because of its efficiency in handling large-scale similarity search and clustering of dense vectors. The process involves the following key steps:

\begin{enumerate}
    \item \textit{Data Preparation:} Initially, we acquire embeddings for our dataset using the pre-trained image and text models.
    
    \item \textit{Index Creation and Configuration:} We use FAISS's \texttt{IndexFlatIP} (Inner Product) index for similarity search in high-dimensional spaces. This index is particularly suited for scenarios where cosine similarity is used (which was the distance metric we used for the contrastive loss function). The dimensionality of the index is set to match that of our embeddings.
    
    \item \textit{Index Population:} The embeddings matrix, an aggregation of individual embeddings obtained from our dataset, is then added to the FAISS index. This allows for efficient storage and retrieval of the embeddings.
    
    \item \textit{Retrieval Process:} During the retrieval phase, for a given query image, its embedding is compared against the indexed embeddings to identify the most similar reports based on the inner product metric. This approach ensures a rapid and accurate retrieval of reports that are most relevant to the input image.
\end{enumerate}

\begin{figure*}
\centerline{\includegraphics[width=1.\textwidth, height=1.04\textheight]{sup_files/context.pdf}}
\caption{A compilation of visual attention maps, corresponding corrections and analytical insights for a selection of test set images.}
\label{fig:attention_maps_all}
\end{figure*}

